The JCMT Gould Belt Survey: radiative heating by OB stars

Radiative feedback can influence subsequent star formation. We quantify the heating from OB stars in the local star-forming regions in the JCMT Gould Belt survey. Dust temperatures are calculated from 450/850 micron flux ratios from SCUBA-2 observations at the JCMT assuming a fixed dust opacity spectral index $\beta=1.8$. Mean dust temperatures are calculated for each submillimetre clump along with projected distances from the main OB star in the region. Temperature vs. distance is fit with a simple model of dust heating by the OB star radiation plus the interstellar radiation field and dust cooling through optically thin radiation. Classifying the heating sources by spectral type, O-type stars produce the greatest clump average temperature rises and largest heating extent, with temperatures over 40 K and significant heating out to at least 2.4 pc. Early-type B stars (B4 and above) produce temperatures of over 20 K and significant heating over 0.4 pc. Late-type B stars show a marginal heating effect within 0.2 pc. For a given projected distance, there is a significant scatter in clump temperatures that is due to local heating by other luminous stars in the region, projection effects, or shadowing effects. Even in these local, `low-mass' star-forming regions, radiative feedback is having an effect on parsec scales, with 24% of the clumps heated to at least 3 K above the 15 K base temperature expected from heating by only the interstellar radiation field, and a mean dust temperature for heated clumps of 24 K.

==> README <==
This directory contains the following source files

LaTeX source:
OBheating.tex
table1.tex   - \include for Table 1

Bibliography:
OBheating.bbl  
OBheating.bib

Figures:
fig1.pdf      fig3.pdf      
fig2.pdf      fig4.pdf

JH 7 May 2021
